CrashFormer: A Multimodal Architecture to Predict the Risk of Crash

Reducing traffic accidents is a crucial global public safety concern. Accident prediction is key to improving traffic safety, enabling proactive measures to be taken before a crash occurs, and informing safety policies, regulations, and targeted interventions. Despite numerous studies on accident prediction over the past decades, many have limitations in terms of generalizability, reproducibility, or feasibility for practical use due to input data or problem formulation. To address existing shortcomings, we propose CrashFormer, a multi-modal architecture that utilizes comprehensive (but relatively easy to obtain) inputs such as the history of accidents, weather information, map images, and demographic information. The model predicts the future risk of accidents on a reasonably acceptable cadence (i.e., every six hours) for a geographical location of 5.161 square kilometers. CrashFormer is composed of five components: a sequential encoder to utilize historical accidents and weather data, an image encoder to use map imagery data, a raw data encoder to utilize demographic information, a feature fusion module for aggregating the encoded features, and a classifier that accepts the aggregated data and makes predictions accordingly. Results from extensive real-world experiments in 10 major US cities show that CrashFormer outperforms state-of-the-art sequential and non-sequential models by 1.8% in F1-score on average when using ``sparse'' input data.

==> tex/ack.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
% \begin{acks}
% To Robert, for the bagels and explaining CMYK and color spaces.
% \end{acks}

==> tex/analysis.tex <==
\section{Data Analysis}
To find out a meaningful correlation among the features and the accidents, an analysis is driven over the dataset. To be able to create a single dataset of accidents, it is necessary to have some assumptions for merging complementary datasets into the accident dataset. For example, to merge a weather event it is supposed that if an event happens, the effects of that can remain up to eight hours after starting of that event.

\subsection{Weather}
As mentioned above, eight backward lookup hours is applied to the weather dataset and the number of weather events is added as separate features for each accident record. The linking feature between the accident and the weather dataset is \textit{AirportCode} that is existing in both datasets and is related to the nearest airport to the accident location.

\subsection{Demographic}
Using the \textit{ZIP Code} information existing in the accident and the socioeconomic dataset, the latter is merged into the former. This joining, provides about 150 new features to the accident dataset.


\subsection{Research gap (Traffic safety equity)}

The current literature provides evidence for the existence of disparities in the incidence and severity of traffic accidents in the United States \citeN{stoker2015pedestrian}. However, most studies examine traffic accident outcomes at metropolitan and census tract scale. This study distinguishes itself by exploring not only the role of traditional traffic exposure factors, built environment risk factors, roadway factors and accident record factors but also the role of social equity measures like race and income in traffic accident outcomes such as accident incidences and severity levels at street segment level using “US-Accidents” dataset that covers 49 contiguous States in the United States over a period of 6 years (2016-2021) \citeN{moosavi2019accident}. 

\subsection{Objectives (Traffic safety equity)}

This study investigates the factors that contribute to traffic accident outcomes like severity and incidence rates within wider socio-economic and demographic context.

\subsection{Implication (Traffic safety equity)}

This study contributes to understanding of the collective influence of traffic exposure factors, roadway factors, built environment features, accident record factors as well as disparate traffic accident severity levels and incidences for different socio-economic groups at street segment level. In addition, findings from this study will help inform policies aimed at addressing traffic exposure, built environment and accident record risk factors as well as the disparate impacts of traffic accident outcomes such as severity levels and incidence rates across different racial and socio-economic groups.



\subsection{Exploratory Data Analysis}

In the exploratory data analysis section, we draw upon five attributes from US-Accidents dataset: traffic exposure factors, built environment risk factors, roadway factors, accident record factors and socio-demographic risk factors. First, we identify top 20 states by accident from among 49 contiguous States. Next, California, Florida, Texas, New York, Pennsylvania, Michigan and Ohio are chosen for further analysis based on traffic exposure factors such as hotspot segment length and points-of-interest (POI), built environment risk factors like population density, roadway factors such as functional classification of road and speed, accident record factors as measured by weather, and socio-demographic risk factors such as income and race.


The study areas represent different land-use, socio-economic and demographic contexts in the United States. Population density is an important indicator for built environment risk factors while median household income is a key metric in traffic safety equity studies. Average population density ranges from 4796, 3431, 2600, 14505, 2490, 2554 to 3840 people per square mile in California, Florida, Michigan, New York, Ohio, Pennsylvania and Texas respectively compared to the average population density of all study areas at 4,530 people per square mile. Furthermore, the average median household income is USD 63, 227 in California; USD 47,351 in Florida; USD 43, 846 in Michigan; USD 70,352 in New York; USD 45, 708 in Ohio; USD 62,449 in Pennsylvania; and USD 51, 361 in Texas compared to the combined average median household income of USD 57, 025 for the seven States.


The weekly, hourly and monthly distribution of traffic accidents are generated in order to make sense of the overall pattern, location and spread characteristics of the data. In our data, traffic event counts are replaced by normalized counts of accidents in States. The range of values are broken down into classes: traffic accident counts are spread from 0 to 24 hours a day, 1 to 7 days a week and 1 to 12 months a year. Peak hourly distribution occurs between 5 and 10, peak weekly distribution occurs on Fridays and peak monthly distribution occurs in December.


The role of traffic exposure factors like length of road extent affected by accidents and road environment features in traffic accident outcomes are analyzed based on hotspot segment length and points-of-interest (POI) attribute in our dataset. 99 percent of the length of road extent affected by accidents is less than 5 miles and accident severity levels vary across space, with accident severity Level 1 influencing hotspot segment lengths less than 30 miles. Furthermore, most accidents occur as a result of lane closures in all States except Texas where accidents occur due to traffic signal. Other points-of-interests that are hotspot for traffic accidents include crossings, road closure points, transit stations, amenities, railways and stations.


As for built environment risk factors, there are obvious differences among accident severity levels with respect to the median population density. Accident severity Level 3 has the highest population density. There is an exponential relationship between population density and traffic accident incidents. As population density increases linearly, traffic accidents decrease exponentially. This association between density and traffic accident severity lends support to another study by (Merlin et al., 2020) who suggest, in their literature review, that accidents that occur in areas of high density are less severe.


Regarding roadway factors, overwhelming majority of accidents occur on motorways with high speed limits, followed by residential, secondary, primary, service and trunk roads. This pattern is linked to the speed of these roads. Motorways have median speed well above 20 miles per hour pedestrian roads that are less prone to accidents have median speed limits below 10 miles per hour.


With respect to accident record factors, most accidents occur during fair weather condition, followed by clear, cloudy and overcast conditions. The higher frequency of accidents in fair weather condition could be attributed to the propensity of the drivers to speed when the weather is good. There is no noticeable difference in the median temperature across the four classes of accident severity. Less severe accidents Level 1 has the highest median temperature, implying that Level 1 accidents are common during hot weather conditions. Additionally, accident severity levels exhibit differences in humid conditions, with accident severity levels increasing with the median value for humidity.


In the exploratory data analysis, disparities in traffic accident outcomes are also analyzed within wider socio-economic and demographic context. Race and income are particularly incorporated into this study because Black, Indigenous and People of Color (BIPOC) are often deprived of access to economic opportunities, and low-income people rely on less costly travel modes such as walking and cycling which increase their exposure to traffic accidents \citeN{roll2021understanding}. The results from this analysis shows that Black, American Indian or Alaskan Native live in areas that experience more severe accidents compared to White neighborhoods which see no difference in the levels of accident severity. This is in line with a previous research (Smart Growth America \& National Complete Streets Coalition, 2019; Schneider, 2020) \citeN{chneider2020united, merlin2020residential} that found areas with a higher proportion of Black or African American and American Indian or Alaska Native residents experience more severe traffic accidents. 
